Stochastic Programming for Dynamic Temperature Control of Refrigerated Road Transport

Temperature control in refrigerated delivery vehicles is critical for preserving product quality, yet existing approaches neglect critical operational uncertainties, such as stochastic door opening durations and heterogeneous initial product temperatures. We propose a framework to optimize cooling policies for refrigerated trucks on fixed routes by explicitly modeling these uncertainties while capturing all relevant thermodynamic interactions in the trailer. To this end, we integrate high-fidelity thermodynamic modeling with a multistage stochastic programming formulation and solve the resulting problem using stochastic dual dynamic programming. In cooperation with industry partners and based on real-world data, we set up computational experiments that demonstrate that our stochastic policy consistently outperforms the best deterministic benchmark by 35% on average while being computationally tractable. In a separate analysis, we show that by fixing the duration of temperature violations, our policy operates with up to $40$\% less fuel than deterministic policies. Our results demonstrate that pallet-level thermal status information is the single most crucial information in the problem and can be used to significantly reduce temperature violations. Knowledge of the timing and length of customer stops is the second most important factor and, together with detailed modeling of thermodynamic interactions, can be used to further significantly reduce violations. Our analysis of the optimal stochastic cooling policy reveals that preemptive cooling before a stop is the key element of an optimal policy. These findings highlight the value of sophisticated control strategies in maintaining the quality of perishable products while reducing the carbon footprint of the industry and improving operational efficiency.

==> draft_old_thermodynamic_models.tex <==
\rpcomm{Old version of the thermodynamic model.}
\begin{align}\label{eq:energy_balance}
  \tilde{C}\left(\ttruck_{i+1} - \ttruck_{i}\right) = \left(\til{h}\til{A}\left(\tamb_i - \ttruck_i\right) + \sum_{p \in P}h_pA_p\left(\ttruck_i - \tprod_{pi}\right) + \heatcu\right)\delta_i
\end{align}
The left-hand side of equation \eqref{eq:energy_balance} is the energy needed to bring $\ttruck_i$ to $\ttruck_{i+1}$ (units: \unit{\joule\per\kg\per\kelvin} $\times$ \unit{\kelvin}). Because of energy conservation, this is equal to the heat (unit \unit{\watt}, i.e. power) transfer between $\tamb_i$ and $\ttruck_i$, plus the heat transfer between  $\ttruck_i$ and the products, i.e., $\tprod$, $p \in P$, plus the heat released by the cooling units multiplied by the time duration $\delta_i$. 

==> parts.tex <==
%%% OLD Case Study Section
\rpcomment{OLD}
Three Dutch companies also contributed to this study by providing practical considerations and real data on which to test the algorithms. Mandersloot is a third-party logistics company (3PL), service providers that handle various supply chain functions for businesses. They own a fleet of dozens of refrigerated trailers that travel daily across different countries in Europe. Tcomm Telematics supplies an accurate online trailer monitoring system for temperature registration and location determination, suitable for every load carrier. With wireless sensors, the transport conditions of Mandersloot trailers are registered and monitored 24/7 via one user-friendly web portal. Their data collection system has been particularly useful because it allows to trace the duration of door openings to each specific customer location. Finally Ortec, offers decision support software and data science expertise to optimize Mandersloot's refrigerated vehicle routes. Their databases did not contain data on the actual door opening time at a customer location, but information on the types of products transported and quantities loaded and unloaded at each stop. This information proved particularly useful for the sample generation phase for the stochastic process.


%%% Old Instance generation section (4.1)
\rpcomment{OLD }
Thanks to this cooperation, we were able to access information on the routes traveled, as well as data on the technical characteristics of the refrigerated vehicles, including size, load capacity, and refrigeration unit performance, which we used to generate the initial instances. Therefore, we reconstructed four routes that were traveled between May 30 and June 1, 2023, identified as MS-469, MS-479, POJ-03, and PZ-734PS. These routes serve as the foundation for our case study, with their principal characteristics summarised in Table \ref{tab:Routes-details}.

In addition to route data, numerous parameters were evaluated to represent the thermodynamic behavior of the system. The following list shows the main categories of parameters along with their references:

\begin{itemize}
    \item Meteorological Variables: data pertaining to typical meteorological patterns for June in the Netherlands were procured from the 'Buienradar' application, ensuring a realistic environmental context for the simulations.
    \item Thermophysical Properties of Air: air properties, pivotal for thermodynamic calculations, were based on data from \cite{CuriosityFluids} website.
    \item Compartment and Refrigeration Unit Specifications: Detailed specifications regarding the cargo compartment dimensions and the refrigeration unit's capacity were furnished by Mandersloot. Furthermore, the thermal transmittance of the compartment walls was suggested by the work of \cite{tassou2009food}.
    \item Energy-to-Fuel Conversion Metrics: The conversion parameters pivotal for translating the refrigeration unit's energy consumption into equivalent fuel usage were derived from the study conducted by \cite{stellingwerf2018reducing}, useful for energy efficiency assessment.
    \item Product-Specific Thermal Parameters: Given the perishable nature of the goods, meat was selected as the transported product category due to its well-documented thermal attributes. The heat transfer coefficient of beef under refrigerated conditions was adopted from \cite{kondjoyan2006review} and the specific heat referenced from \cite{TheEngineeringToolBox}. 
    To ensure adherence to safety standards, the storage temperature was set within the optimal range of 0.85 $^\circ$C to 3.85 $^\circ$C.
    \item pallet characteristics: standard euro-pallet dimensions.
\end{itemize}

% old Myopic description
\begin{comment} 
$$O_i^{H1}=\begin{cases} 1, & \text{ if } \max_{p \in \Pc_i} T_{pi} - \bar T_p > \lambda_1^{H1} \text{ or } \ttruck_i > \min_{p \in \Pc_i} \bar T_p \\ 1, & \text{ if } O_{i-1}^{H1} = 1 \text{ and } \min_{p \in \Pc_i} \underline{T}_p - T_{pi} > \lambda_2^{H1}  \\ 0, & \text{ otherwise }  \end{cases}$$
    
\subsection{A Simple Heuristic}
A heuristic policy that we refer as Myopic emulates the common approach taken by the on–off feedback controller with hysteresis of cooling systems \citep{li2010optimal}. Thus, this strategy provides a suitable basis for comparison because of its simplicity and common application. Operationally, it consists of maintaining the internal temperature within a specific range by switching the system on or off \citep{HUANG2017576}. Specifically, this strategy involves operating the cooling unit at full capacity when the internal temperature reaches the upper allowable limit and turning it off when it falls below the lower limit. The amplitude and frequency characteristics of the temperature oscillation cycles influence the system performance criteria including: temperature deviations, mechanical component wear and energy consumption. In particular, experiments have pointed out the inability of this method to keep products within the ideal temperature range, mainly due to its reactive nature.
    
To address this problem, we enhanced the policy by introducing a parameter, $\lambda$, ranging from 0 to 1. This parameter determines the specific temperature point between the upper and lower limits at which the cooling unit is activated. By adjusting $\lambda$, we can balance the cooling unit's operation: a lower $\lambda$ value means the unit operates more frequently, thereby reducing temperature deviations. However, excessively low values can lead to impractically high cooling unit cycle rates, causing excessive wear of mechanical components over time. Therefore, we set $\lambda$ to 0.5, which we found to be a reasonable compromise between performance and practicality.
This policy still has a significant disadvantage compared to RLP and SDDP. In addition to lacking any information about future conditions, its decisions are based solely on the indoor air temperature. To explore whether incorporating the temperature state of the products could provide additional value, we implemented two alternative policies: Peak Temp Policy (PTP) and Average Temp Policy (ATP). Both of these policies build upon the standard myopic approach but include additional knowledge about the temperature of the products at each time period. Specifically:
\begin{itemize}
    \item PTP: This policy activates the refrigeration unit when the temperature of the hottest product exceeds the allowable range and keeps it on until that product returns to the mid-range.

    \item ATP: This policy, instead, considers the average temperature of the products and turns the unit on whenever this value exceeds the allowable range, keeping it active until the average temperature returns to mid-range.
\end{itemize}
To ensure that decisions do not conflict, the cooling unit remains active as long as any control criterion (air temperature or product temperature) dictates the need for cooling. The unit is turned off only when neither control system signals the need to keep it running.

%\item Possibly prove that the myopic policy always uses the least fuel.
\end{comment}




%%%%%%%%%%%%%%%%%%%%%%%
%%% 1. Introduction %%%
%%%%%%%%%%%%%%%%%%%%%%%

% Temperature-regulated supply chains, often referred to as \emph{cold chains}, are central to agribusiness logistics and the pharmaceutical sector. Valued at \$313.3 billion in 2024 and projected to reach \$410.7 billion by 2028, the global cold chain logistics market is experiencing significant growth, mainly due to globalization and the expansion of e-commerce \citep{statista, song2022research}. This growth has led to longer and more complex logistics processes, along with the challenges of maintaining cargo storage within specific temperature and humidity conditions at each stage of the chain. As one of the major components of cold chains, refrigerated transport systems are attracting more and more interest due to ever-increasing expectations in terms of quality and safety of the transported perishable goods, as well as considerable energy consumption \citep{li2012dynamic, tassou2009food}. Effective temperature control and reliable monitoring technology are crucial aspects of these systems to preserve product shelf life and meet regulatory standards. According to \cite{rong2011optimization, hsu2007vehicle}, temperature represents the main environmental factor leading to quality degradation of the food products.
% To this end, refrigerated road vehicles are commonly equipped with a vapor compression cycle system (hereafter referred to as cooling unit) to regulate internal temperature and possibly keep it within an allowable range \citep{li2010optimal}. The unit works by absorbing heat from the refrigerated cargo space and transferring it to the surroundings by repetitive cycling of a refrigerant between two heat exchangers, that is, an evaporator and a condenser (see \cite{larsen2007potential} for more details). The most commonly used temperature regulation approach in refrigerated transport systems is known as on-off feedback controller with hysteresis. According to this control scheme, the unit is activated and deactivated based on the difference between the measured cargo space temperature and temperature set-point \citep{li2010optimal, HUANG2017576}. 

% Despite advancements in equipment, the risk of product spoilage due to insufficient refrigeration is significant \citep{aiello2012simulation, konovalenko2021real}. This issue is particularly severe during the distribution phase, where perishable products are delivered using specialized vehicles that visit several customers. During this process, operators must frequently open the vehicle doors, resulting in significant heat infiltration from the outside which inevitably leads to quality loss \citep{tassou2009food}. In contrast to stationary systems, transport refrigeration systems are subjected to more demanding operating conditions, such as the wide diversity of products loaded and variations in weather conditions \citep{li2012dynamic, tassou2009food}. Current control schemes operate according with a purely reactive and myopic rule, disregarding several variables essential for supporting preventive cooling decisions that could significantly reduce the risk of both food and energy waste. These variables include route-related information, such as environmental conditions, specific product requirements, travel times, and customer stops, which inevitably represent significant sources of uncertainty. In addition, refrigeration is well known to be one of the largest energy consumers worldwide \citep{larsen2007potential} and due to that, cold chain operations, including transportation, currently contribute $1\%$ of global GHG emissions \citep{taher2021thermal}. Refrigeration trucks are commonly equipped with diesel engine-driven refrigeration units, which is why their fuel consumption can be up to one-and-a-half times higher than their non-refrigerated counterpart \citep{deng2023pickup, song2022research}, making temperature controlled delivery the most energy-consuming kind of road freight transport \citep{de2015experimental}.

% These figures underscore the severe implications of the cold chain for the food waste and the environment, enhancing the requirement for innovative control approaches \citep{li2010optimal, song2022research}, as well as technical and planning solutions that facilitate efficient and sustainable transport operations \citep{akkacs2022om, hillier2015introduction}.
